Exploring the Use of Static and Dynamic Analysis to Improve the Performance of the Mining Sandbox Approach for Android Malware Identification

The Android mining sandbox approach consists in running dynamic analysis tools on a benign version of an Android app and recording every call to sensitive APIs. Later, one can use this information to (a) prevent calls to other sensitive APIs (those not previously recorded) or (b) run the dynamic analysis tools again in a different version of the app -- in order to identify possible malicious behavior. Although the use of dynamic analysis for mining Android sandboxes has been empirically investigated before, little is known about the potential benefits of combining static analysis with the mining sandbox approach for identifying malicious behavior. As such, in this paper we present the results of two empirical studies: The first is a non-exact replication of a previous research work from Bao et al., which compares the performance of test case generation tools for mining Android sandboxes. The second is a new experiment to investigate the implications of using taint analysis algorithms to complement the mining sandbox approach in the task to identify malicious behavior. Our study brings several findings. For instance, the first study reveals that a static analysis component of DroidFax (a tool used for instrumenting Android apps in the Bao et al. study) contributes substantially to the performance of the dynamic analysis tools explored in the previous work. The results of the second study show that taint analysis is also practical to complement the mining sandboxes approach, improve the performance of the later strategy in at most 28.57%.

==> flowdroid.tex <==
\section{Flowdroid for static analysis}
